Generating Wikipedia by Summarizing Long Sequences

We show that generating English Wikipedia articles can be approached as a multi- document summarization of source documents. We use extractive summarization to coarsely identify salient information and a neural abstractive model to generate the article. For the abstractive model, we introduce a decoder-only architecture that can scalably attend to very long sequences, much longer than typical encoder- decoder architectures used in sequence transduction. We show that this model can generate fluent, coherent multi-sentence paragraphs and even whole Wikipedia articles. When given reference documents, we show it can extract relevant factual information as reflected in perplexity, ROUGE scores and human evaluations.

==> ex_perfrep.tex <==
\model-wiki-input-cap{`` perfect replacement '' is a song by english electronic music duo example . it was released as the lead single from their third studio album , the evolution of man ( 2012 ) . the song peaked at number one on the uk singles chart and number one on the irish singles chart . }
{`` perfect replacement '' is a song by british recording artist example . it was released as the third single from his fourth studio album , the evolution of man , on 24 february 2013 following his uk arena tour . the song was written by elliot gleave and feed me , the latter who also produced the song .}
{Perfect Replacement<EOT>this is an audio clip for ' perfect replacement ' premiered by greg james on bbc radio 1 on thursday 15th november 2012 . produced by feed me , ' perfect replacement ' is taken from example 's new album ' the evolution of man ' ( out now ) . creating pixel - perfect art in illustrator is now easier and more intuitive than ever before . draw pixel - perfect art that looks sharp and crisp on screens at different stroke widths and alignment options . choose to align an existing object to the pixel grid with a single click or align a new object right while drawing it . while transforming objects , you can preserve pixel - alignment without distorting the artwork . pixel - alignment works for objects as well as individual path segments and anchor points that comprise them . i just opened the package yesterday . i wanted them to replace my spin for perfect skin brushes . they are not as good quality . will not order again , will only replace my brushes with spin for perfect skin brushes . the brushes seem stiffer , also . example -- ' perfect replacement ' ( official video ) - capital example -- ' perfect replacement ' ( official video ) example has released the official video to his latest single ' perfect replacement ' , which is the latest to be taken from fourth album ' the evolution of man ' . check out the official video to example 's new song ' perfect replacement ' below : example - perfect replacement ( datsik remix ) example -- perfect replacement ( datsik remix ) is released 24th february on ministry of sound . judging by the newies he shows off here , he might just go further and all . besides single ' say nothing 's coldplay - thieving ` whooaaas '' , ' close enemies ' is a shady , trance anthem with a stadium - kind chorus ; ' perfect replacement ' recalls the sharpest beats of the prodigy by way of a riff you 'd find on guitar hero 's toughest level . example -- perfect replacement ( r3hab \& hard rock sofa remix ) mixjunkies earlier this year , example released a brand new album that rocked the world . the evolution of man was an album that was produced by some of the biggest names in music and received great reviews from critics around the world . this author being a huge fan of it . now example is set to release his third single off of that album ' perfect replacement ' . the package is going to have remixes from datsik , r3hab \& hard rock sofa , toyboy \& robin and danny howard . today we have a preview of the r3hab and hard rock sofa remix of the track . it features the giant chainsaw sound that r3hab is so well known for while bringing in the big room synths and epic melodies . check out the remix right here . the single is going to be released on february 24 of the new year and expect the music video soon as it just finished filming on december 11 . example - perfect replacement ( danny howard remix ) ( ministry of sound tv ) - youtube this is danny howard 's remix of example ' perfect replacement ' on ministry of sound tv , the best in new dance music . make sure you subscribe and follow us online at the links below ! example also revealed that ' say nothing ' and ' perfect replacement ' will receive their live debuts when he performs at v festival on august 18 and 19 . the rapper is currently shooting the video for ' say nothing ' in the spanish desert . linking to an instagram picture of the set 's sunny location , he noted : ` it 's so hot here you could cook a steak on your own forehead . '' example - ' perfect replacement ' ( r3hab \& hard rock sofa extended vocal mix ) ( ministry of sound tv ) - youtube this is r3hab \& hard rock sofa 's remix of example ' perfect replacement ' on ministry of sound tv , the best in new dance music . make sure you subscribe and follow us online at the links below ! example - ' perfect replacement ' ( audio only ) - youtube download the ' perfect replacement ' ep on itunes ( out now ) : http://www.smarturl.it/perfectreplace ... example lyrics - perfect replacement ` perfect replacement '' lyrics example lyrics are property and copyright of their owners . ` perfect replacement '' lyrics provided for educational purposes and personal use only . example -- perfect replacement lyrics genius lyrics perfect replacement perfect replacement lyrics example - perfect replacement lyrics metrolyrics perfect replacement , a song by example}
{Caption bengali :}

